Are generative deep models for novelty detection truly better?

Many deep models have been recently proposed for anomaly detection. This paper presents comparison of selected generative deep models and classical anomaly detection methods on an extensive number of non--image benchmark datasets. We provide statistical comparison of the selected models, in many configurations, architectures and hyperparamaters. We arrive to conclusion that performance of the generative models is determined by the process of selection of their hyperparameters. Specifically, performance of the deep generative models deteriorates with decreasing amount of anomalous samples used in hyperparameter selection. In practical scenarios of anomaly detection, none of the deep generative models systematically outperforms the kNN.

==> misc/aaucsummary.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c | c c c c c c } 
    & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  test auc & 4.26 & 5.90 & 3.54 & 2.20 & 3.56 & 1.54  \\ 
  train auc & 3.19 & 5.39 & 3.71 & 3.21 & 3.70 & 1.80  \\ 
  top 5\% & 2.56 & 5.01 & 3.14 & 2.67 & 4.53 & 3.09  \\ 
  top 1\% & 2.20 & 4.59 & 3.21 & 2.71 & 4.47 & 3.81  \\ 
 \end{tabular}
 \caption{Average ranks of algorithms for different hyperparameter selection criteria using the augmented AUROC.} 
 \label{tab:aaucsummary} 
\end{table}

==> misc/ftfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 0.12(1.0) & 0.46(2.0) & 28.75(3.0) & 165.58(6.0) & 86.70(4.0) & 108.74(5.0)  \\ 
  blo & 0.03(1.0) & 0.31(2.0) & 21.42(3.0) & 119.27(6.0) & 68.44(4.0) & 80.90(5.0)  \\ 
  brc & 0.04(1.0) & 0.30(2.0) & 59.20(3.0) & 325.35(6.0) & 149.46(4.0) & 198.93(5.0)  \\ 
  brt & 0.03(1.0) & 0.24(2.0) & 13.79(3.0) & 84.57(6.0) & 49.86(4.0) & 58.17(5.0)  \\ 
  car & 0.04(1.0) & 0.39(2.0) & 55.27(3.0) & 308.92(6.0) & 142.17(4.0) & 187.20(5.0)  \\ 
  eco & 0.03(1.0) & 0.27(2.0) & 20.02(3.0) & 119.25(6.0) & 65.25(4.0) & 79.14(5.0)  \\ 
  gla & 0.00(1.0) & 0.25(2.0) & 17.33(3.0) & 104.83(6.0) & 58.84(4.0) & 71.10(5.0)  \\ 
  hab & 0.03(1.0) & 0.28(2.0) & 16.90(3.0) & 98.66(6.0) & 57.22(4.0) & 66.27(5.0)  \\ 
  ion & 0.04(1.0) & 0.28(2.0) & 49.83(3.0) & 276.94(6.0) & 127.92(4.0) & 169.65(5.0)  \\ 
  iri & 0.00(1.0) & 0.26(2.0) & 13.33(3.0) & 78.78(6.0) & 47.62(4.0) & 54.32(5.0)  \\ 
  iso & 1.50(1.0) & 1.74(2.0) & 2154.48(3.0) & 7277.27(6.0) & 6577.41(5.0) & 6368.50(4.0)  \\ 
  let & 1.00(1.0) & 1.66(2.0) & 2146.91(3.0) & 7266.16(6.0) & 6539.56(5.0) & 6340.14(4.0)  \\ 
  lib & 0.06(1.0) & 0.27(2.0) & 115.67(3.0) & 716.92(6.0) & 284.56(4.0) & 372.85(5.0)  \\ 
  mad & 0.49(1.0) & 0.57(2.0) & 1465.07(3.0) & 6090.18(6.0) & 5119.09(5.0) & 5054.86(4.0)  \\ 
  mag & 0.01(1.0) & 0.96(2.0) & 29.16(3.0) & 167.57(6.0) & 86.35(4.0) & 109.60(5.0)  \\ 
  min & 0.34(1.0) & 7.34(2.0) & 92.92(3.0) & 507.88(6.0) & 217.46(4.0) & 293.05(5.0)  \\ 
  mul & 0.70(2.0) & 0.64(1.0) & 2351.73(3.0) & 7606.64(6.0) & 7057.55(5.0) & 6945.77(4.0)  \\ 
  mus & 0.20(1.0) & 0.95(2.0) & 310.25(3.0) & 2674.09(6.0) & 903.97(4.0) & 1701.46(5.0)  \\ 
  pag & 0.06(1.0) & 0.53(2.0) & 27.95(3.0) & 166.83(6.0) & 85.09(4.0) & 109.05(5.0)  \\ 
  par & 0.03(1.0) & 0.26(2.0) & 27.96(3.0) & 167.55(6.0) & 82.22(4.0) & 105.84(5.0)  \\ 
  pen & 0.05(1.0) & 0.61(2.0) & 37.52(3.0) & 221.33(6.0) & 105.02(4.0) & 136.76(5.0)  \\ 
  pim & 0.03(1.0) & 0.32(2.0) & 24.31(3.0) & 152.33(6.0) & 79.90(4.0) & 99.52(5.0)  \\ 
  son & 0.04(1.0) & 0.25(2.0) & 47.75(3.0) & 259.92(6.0) & 124.95(4.0) & 162.94(5.0)  \\ 
  spe & 0.04(1.0) & 0.26(2.0) & 58.73(3.0) & 324.88(6.0) & 146.31(4.0) & 198.55(5.0)  \\ 
  ssa & 0.05(1.0) & 0.50(2.0) & 68.57(3.0) & 379.47(6.0) & 169.28(4.0) & 227.38(5.0)  \\ 
  sse & 0.04(1.0) & 0.37(2.0) & 40.46(3.0) & 237.17(6.0) & 112.29(4.0) & 146.65(5.0)  \\ 
  ssh & 0.03(1.0) & 3.40(2.0) & 25.63(3.0) & 152.13(6.0) & 79.54(4.0) & 100.74(5.0)  \\ 
  sve & 0.00(1.0) & 0.33(2.0) & 41.04(3.0) & 237.22(6.0) & 112.38(4.0) & 147.00(5.0)  \\ 
  syn & 0.00(1.0) & 0.31(2.0) & 104.64(3.0) & 624.70(6.0) & 246.84(4.0) & 341.28(5.0)  \\ 
  ver & 0.03(1.0) & 0.30(2.0) & 21.45(3.0) & 135.84(6.0) & 71.64(4.0) & 90.08(5.0)  \\ 
  wal & 0.04(1.0) & 0.46(2.0) & 49.51(3.0) & 279.51(6.0) & 130.75(4.0) & 173.40(5.0)  \\ 
  wa1 & 0.04(1.0) & 0.47(2.0) & 45.64(3.0) & 259.11(6.0) & 122.29(4.0) & 160.91(5.0)  \\ 
  wa2 & 0.00(1.0) & 0.47(2.0) & 46.08(3.0) & 255.54(6.0) & 122.16(4.0) & 161.59(5.0)  \\ 
  win & 0.03(1.0) & 0.26(2.0) & 17.73(3.0) & 114.57(6.0) & 60.39(4.0) & 75.16(5.0)  \\ 
  yea & 0.00(1.0) & 0.33(2.0) & 24.48(3.0) & 147.97(6.0) & 78.62(4.0) & 100.45(5.0)  \\ 
  \hline
  avg & 0.15(1.03) & 0.76(1.97) & 276.33(3.0) & 1088.71(6.0) & 844.83(4.11) & 879.94(4.89)  \\ 
 \end{tabular}
 }
 \caption{Mean fit times over datasets with ranks and average} 
 \label{tab:ftfull} 
\end{table}

==> misc/ptfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 0.04(1.0) & 0.30(2.0) & 1.02(3.0) & 1.16(4.0) & 1.87(5.0) & 2.02(6.0)  \\ 
  blo & 0.00(1.0) & 0.13(2.0) & 1.12(6.0) & 0.24(3.0) & 0.39(5.0) & 0.35(4.0)  \\ 
  brc & 0.01(1.0) & 0.13(2.0) & 0.55(6.0) & 0.22(3.0) & 0.36(4.5) & 0.36(4.5)  \\ 
  brt & 0.00(1.0) & 0.11(5.0) & 0.47(6.0) & 0.05(2.0) & 0.10(4.0) & 0.07(3.0)  \\ 
  car & 0.08(1.0) & 0.23(2.0) & 0.92(3.0) & 1.03(4.0) & 1.67(5.0) & 1.80(6.0)  \\ 
  eco & 0.00(1.0) & 0.12(2.0) & 0.59(6.0) & 0.13(3.0) & 0.22(5.0) & 0.20(4.0)  \\ 
  gla & 0.00(1.0) & 0.11(3.0) & 0.41(6.0) & 0.08(2.0) & 0.13(5.0) & 0.12(4.0)  \\ 
  hab & 0.00(1.0) & 0.12(2.0) & 0.94(6.0) & 0.14(3.0) & 0.26(5.0) & 0.21(4.0)  \\ 
  ion & 0.00(1.0) & 0.13(2.5) & 0.47(6.0) & 0.13(2.5) & 0.24(5.0) & 0.23(4.0)  \\ 
  iri & 0.00(1.0) & 0.11(4.0) & 0.94(6.0) & 0.07(2.0) & 0.14(5.0) & 0.10(3.0)  \\ 
  iso & 5.77(4.0) & 0.95(1.0) & 3.83(2.0) & 4.75(3.0) & 17.75(6.0) & 10.73(5.0)  \\ 
  let & 4.98(4.0) & 0.91(1.0) & 3.61(2.0) & 4.42(3.0) & 16.56(6.0) & 9.94(5.0)  \\ 
  lib & 0.01(1.0) & 0.13(2.5) & 0.46(6.0) & 0.13(2.5) & 0.22(4.0) & 0.24(5.0)  \\ 
  mad & 0.33(2.0) & 0.32(1.0) & 1.21(4.0) & 1.17(3.0) & 4.15(6.0) & 2.83(5.0)  \\ 
  mag & 0.99(2.0) & 0.89(1.0) & 3.82(3.0) & 6.62(4.0) & 10.81(5.0) & 11.87(6.0)  \\ 
  min & 151.31(6.0) & 7.27(1.0) & 28.36(2.0) & 52.72(3.0) & 85.12(4.0) & 93.26(5.0)  \\ 
  mul & 0.36(2.0) & 0.35(1.0) & 1.00(3.0) & 1.33(4.0) & 5.01(6.0) & 3.04(5.0)  \\ 
  mus & 2.03(2.0) & 0.67(1.0) & 2.21(3.0) & 3.28(4.0) & 6.18(5.0) & 6.73(6.0)  \\ 
  pag & 0.22(1.0) & 0.39(2.0) & 1.37(3.0) & 2.64(4.0) & 4.28(5.0) & 4.69(6.0)  \\ 
  par & 0.00(1.0) & 0.11(4.0) & 0.05(2.0) & 0.09(3.0) & 0.14(5.0) & 0.15(6.0)  \\ 
  pen & 0.29(1.0) & 0.49(2.0) & 1.55(3.0) & 3.02(4.0) & 4.88(5.0) & 5.35(6.0)  \\ 
  pim & 0.01(1.0) & 0.14(2.0) & 0.15(3.0) & 0.27(4.0) & 0.46(5.0) & 0.48(6.0)  \\ 
  son & 0.00(1.0) & 0.11(4.5) & 0.04(2.0) & 0.07(3.0) & 0.11(4.5) & 0.12(6.0)  \\ 
  spe & 0.00(1.0) & 0.12(3.5) & 0.06(2.0) & 0.12(3.5) & 0.20(5.0) & 0.21(6.0)  \\ 
  ssa & 0.23(1.0) & 0.35(2.0) & 1.05(3.0) & 2.00(4.0) & 3.25(5.0) & 3.54(6.0)  \\ 
  sse & 0.03(1.0) & 0.20(2.0) & 0.37(3.0) & 0.72(4.0) & 1.17(5.0) & 1.28(6.0)  \\ 
  ssh & 19.84(3.0) & 3.62(1.0) & 14.86(2.0) & 29.32(4.0) & 47.66(5.0) & 51.99(6.0)  \\ 
  sve & 0.01(1.0) & 0.16(2.0) & 0.18(3.0) & 0.34(4.0) & 0.56(5.0) & 0.61(6.0)  \\ 
  syn & 0.01(1.0) & 0.14(3.0) & 0.13(2.0) & 0.22(4.0) & 0.38(5.0) & 0.41(6.0)  \\ 
  ver & 0.00(1.0) & 0.14(3.0) & 0.12(2.0) & 0.22(4.0) & 0.36(5.0) & 0.39(6.0)  \\ 
  wal & 0.14(1.0) & 0.31(2.0) & 0.84(3.0) & 1.56(4.0) & 2.61(5.0) & 2.84(6.0)  \\ 
  wa1 & 0.22(1.0) & 0.33(2.0) & 0.94(3.0) & 1.75(4.0) & 2.95(5.0) & 3.21(6.0)  \\ 
  wa2 & 0.22(1.0) & 0.32(2.0) & 0.94(3.0) & 1.73(4.0) & 2.96(5.0) & 3.22(6.0)  \\ 
  win & 0.00(1.0) & 0.11(5.5) & 0.03(2.0) & 0.06(3.0) & 0.10(4.0) & 0.11(5.5)  \\ 
  yea & 0.01(1.0) & 0.16(2.0) & 0.20(3.0) & 0.39(4.0) & 0.65(5.0) & 0.72(6.0)  \\ 
  \hline
  avg & 5.35(1.49) & 0.58(2.3) & 2.14(3.51) & 3.49(3.41) & 6.40(4.97) & 6.38(5.31)  \\ 
 \end{tabular}
 }
 \caption{Mean predict times over datasets with ranks and average} 
 \label{tab:ptfull} 
\end{table}

==> misc/testaaucfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 3.62(5.0) & 2.43(6.0) & 3.66(4.0) & 3.84(2.0) & 3.73(3.0) & 5.54(1.0)  \\ 
  blo & 4.43(5.0) & 3.94(6.0) & 4.45(4.0) & 4.83(2.0) & 4.54(3.0) & 4.93(1.0)  \\ 
  brc & 3.44(6.0) & 4.38(5.0) & 4.85(1.0) & 4.75(3.0) & 4.55(4.0) & 4.84(2.0)  \\ 
  brt & 3.55(5.5) & 3.55(5.5) & 3.75(2.5) & 3.75(2.5) & 3.75(2.5) & 3.75(2.5)  \\ 
  car & 1.58(5.0) & 1.42(6.0) & 1.82(4.0) & 2.17(3.0) & 2.87(2.0) & 3.28(1.0)  \\ 
  eco & 3.37(5.0) & 2.24(6.0) & 3.84(3.0) & 3.99(2.0) & 3.77(4.0) & 4.25(1.0)  \\ 
  gla & 2.28(5.0) & 1.94(6.0) & 3.49(4.0) & 4.18(2.0) & 4.13(3.0) & 4.23(1.0)  \\ 
  hab & 3.78(3.0) & 3.23(6.0) & 3.74(4.0) & 4.17(2.0) & 3.52(5.0) & 4.34(1.0)  \\ 
  ion & 3.82(5.0) & 3.20(6.0) & 4.25(3.0) & 4.33(2.0) & 4.16(4.0) & 4.34(1.0)  \\ 
  iri & 3.11(5.0) & 2.44(6.0) & 3.55(3.5) & 3.60(1.5) & 3.55(3.5) & 3.60(1.5)  \\ 
  iso & 2.49(2.0) & 1.46(6.0) & 2.34(3.0) & 2.74(1.0) & 1.66(5.0) & 2.29(4.0)  \\ 
  let & 2.50(2.0) & 1.20(6.0) & 2.42(3.0) & 2.80(1.0) & 1.57(5.0) & 2.38(4.0)  \\ 
  lib & 2.35(5.0) & 1.63(6.0) & 2.89(4.0) & 3.91(2.0) & 3.16(3.0) & 4.28(1.0)  \\ 
  mad & 1.29(6.0) & 1.32(5.0) & 1.62(4.0) & 2.00(2.0) & 1.84(3.0) & 4.50(1.0)  \\ 
  mag & 4.72(2.0) & 3.52(6.0) & 4.25(5.0) & 4.51(4.0) & 4.62(3.0) & 6.31(1.0)  \\ 
  min & 3.15(4.0) & 2.30(5.0) & 2.17(6.0) & 3.72(1.0) & 3.21(3.0) & 3.52(2.0)  \\ 
  mul & 4.67(4.0) & 2.19(6.0) & 5.02(3.0) & 5.61(1.0) & 3.61(5.0) & 5.19(2.0)  \\ 
  mus & 5.91(3.0) & 1.22(6.0) & 6.23(2.0) & 6.52(1.0) & 3.10(5.0) & 5.25(4.0)  \\ 
  pag & 4.57(4.0) & 3.68(6.0) & 5.19(3.0) & 5.39(2.0) & 4.43(5.0) & 6.88(1.0)  \\ 
  par & 2.80(5.0) & 2.21(6.0) & 3.63(4.0) & 3.90(3.0) & 4.11(2.0) & 4.34(1.0)  \\ 
  pen & 6.30(1.0) & 2.99(6.0) & 5.47(3.0) & 5.83(2.0) & 4.19(5.0) & 5.23(4.0)  \\ 
  pim & 2.74(5.0) & 2.49(6.0) & 2.95(4.0) & 3.33(3.0) & 3.37(2.0) & 4.81(1.0)  \\ 
  son & 1.59(5.0) & 1.46(6.0) & 2.84(4.0) & 4.18(3.0) & 4.23(1.5) & 4.23(1.5)  \\ 
  spe & 2.64(5.0) & 2.26(6.0) & 3.54(4.0) & 4.30(2.5) & 4.30(2.5) & 4.35(1.0)  \\ 
  ssa & 4.72(5.0) & 3.99(6.0) & 5.04(3.0) & 5.07(2.0) & 4.75(4.0) & 5.52(1.0)  \\ 
  sse & 4.31(4.0) & 2.99(6.0) & 4.55(3.0) & 4.67(2.0) & 4.23(5.0) & 5.36(1.0)  \\ 
  ssh & 6.32(2.0) & 4.06(6.0) & 5.83(4.0) & 5.96(3.0) & 5.07(5.0) & 8.32(1.0)  \\ 
  sve & 2.53(5.0) & 1.98(6.0) & 3.13(4.0) & 3.35(2.0) & 3.22(3.0) & 4.31(1.0)  \\ 
  syn & 4.79(3.5) & 2.91(6.0) & 4.79(3.5) & 5.25(2.0) & 4.41(5.0) & 5.34(1.0)  \\ 
  ver & 2.16(5.0) & 1.98(6.0) & 2.41(4.0) & 3.12(2.0) & 3.06(3.0) & 4.70(1.0)  \\ 
  wal & 2.96(2.0) & 1.75(6.0) & 2.39(4.0) & 2.47(3.0) & 2.32(5.0) & 3.52(1.0)  \\ 
  wa1 & 2.65(5.0) & 2.13(6.0) & 3.53(4.0) & 3.57(3.0) & 4.10(2.0) & 5.08(1.0)  \\ 
  wa2 & 2.53(5.0) & 2.06(6.0) & 3.19(4.0) & 3.40(3.0) & 4.05(2.0) & 5.09(1.0)  \\ 
  win & 3.68(5.0) & 3.36(6.0) & 4.19(2.5) & 4.19(2.5) & 4.19(2.5) & 4.19(2.5)  \\ 
  yea & 2.60(5.0) & 2.10(6.0) & 3.22(3.0) & 3.41(2.0) & 2.94(4.0) & 4.94(1.0)  \\ 
  \hline
  avg & 3.31(4.26) & 2.44(5.9) & 3.18(3.54) & 3.27(2.2) & 2.66(3.56) & 3.16(1.54)  \\ 
 \end{tabular}
 }
 \caption{Augmented AUC scores and ranks using the first hyperparameter selection criterion.} 
 \label{tab:testaaucfull} 
\end{table}

==> misc/top1aaucfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 3.52(1.0) & 2.36(5.0) & 2.82(3.0) & 2.94(2.0) & 1.77(6.0) & 2.45(4.0)  \\ 
  blo & 4.08(1.0) & 3.94(2.0) & 3.50(4.0) & 3.89(3.0) & 3.35(5.0) & 3.27(6.0)  \\ 
  brc & 3.38(4.5) & 4.27(1.0) & 3.38(4.5) & 3.62(2.0) & 3.43(3.0) & 2.58(6.0)  \\ 
  brt & 3.35(3.0) & 3.55(2.0) & 3.60(1.0) & 3.00(4.0) & 2.73(6.0) & 2.78(5.0)  \\ 
  car & 1.58(5.0) & 1.42(6.0) & 1.61(4.0) & 1.66(2.5) & 1.66(2.5) & 1.99(1.0)  \\ 
  eco & 3.26(1.0) & 2.21(6.0) & 2.64(5.0) & 3.08(2.0) & 2.83(3.0) & 2.81(4.0)  \\ 
  gla & 2.23(3.0) & 1.84(6.0) & 2.31(2.0) & 2.05(5.0) & 2.20(4.0) & 2.77(1.0)  \\ 
  hab & 3.45(1.0) & 3.19(2.0) & 2.58(4.0) & 3.06(3.0) & 2.41(5.0) & 2.15(6.0)  \\ 
  ion & 3.74(1.0) & 2.95(4.0) & 3.73(2.0) & 3.51(3.0) & 2.88(5.0) & 2.36(6.0)  \\ 
  iri & 2.91(2.0) & 2.29(6.0) & 2.73(3.0) & 2.61(4.0) & 3.00(1.0) & 2.58(5.0)  \\ 
  iso & 2.49(1.0) & 1.44(5.0) & 2.24(3.0) & 2.28(2.0) & 1.42(6.0) & 1.89(4.0)  \\ 
  let & 2.50(1.0) & 1.18(6.0) & 2.36(3.0) & 2.40(2.0) & 1.28(5.0) & 1.83(4.0)  \\ 
  lib & 2.35(1.0) & 1.56(6.0) & 2.16(3.0) & 1.99(5.0) & 2.00(4.0) & 2.31(2.0)  \\ 
  mad & 1.21(5.0) & 1.25(4.0) & 1.17(6.0) & 1.33(3.0) & 1.37(2.0) & 2.15(1.0)  \\ 
  mag & 4.72(1.0) & 3.49(4.0) & 4.11(3.0) & 4.31(2.0) & 3.08(6.0) & 3.11(5.0)  \\ 
  min & 2.33(4.0) & 2.28(5.0) & 2.00(6.0) & 3.67(1.0) & 2.88(2.0) & 2.81(3.0)  \\ 
  mul & 4.66(2.0) & 2.08(6.0) & 4.57(3.0) & 5.22(1.0) & 2.89(5.0) & 3.02(4.0)  \\ 
  mus & 5.91(1.0) & 1.06(6.0) & 5.69(2.0) & 5.62(3.0) & 2.19(5.0) & 3.98(4.0)  \\ 
  pag & 4.55(3.0) & 3.66(4.0) & 5.03(2.0) & 5.05(1.0) & 3.25(6.0) & 3.49(5.0)  \\ 
  par & 2.80(1.0) & 2.14(5.0) & 2.56(2.0) & 2.30(4.0) & 1.78(6.0) & 2.44(3.0)  \\ 
  pen & 6.30(1.0) & 2.91(6.0) & 4.90(3.0) & 5.26(2.0) & 3.20(4.0) & 2.97(5.0)  \\ 
  pim & 2.47(1.0) & 2.42(2.0) & 2.22(4.0) & 2.41(3.0) & 1.98(5.0) & 1.89(6.0)  \\ 
  son & 1.47(4.0) & 1.43(5.0) & 1.37(6.0) & 1.61(3.0) & 2.01(2.0) & 2.97(1.0)  \\ 
  spe & 2.27(3.0) & 1.97(4.5) & 2.61(1.0) & 2.45(2.0) & 1.95(6.0) & 1.97(4.5)  \\ 
  ssa & 4.72(2.0) & 3.98(5.0) & 3.94(6.0) & 4.15(4.0) & 4.31(3.0) & 4.79(1.0)  \\ 
  sse & 4.31(1.0) & 2.93(6.0) & 3.92(3.0) & 3.88(4.0) & 3.08(5.0) & 3.95(2.0)  \\ 
  ssh & 5.77(2.0) & 3.88(5.0) & 5.69(3.0) & 5.79(1.0) & 2.87(6.0) & 3.90(4.0)  \\ 
  sve & 2.51(2.0) & 1.97(5.0) & 2.55(1.0) & 2.31(4.0) & 1.68(6.0) & 2.34(3.0)  \\ 
  syn & 4.49(1.0) & 2.80(5.0) & 3.81(3.0) & 3.86(2.0) & 2.07(6.0) & 3.14(4.0)  \\ 
  ver & 1.14(6.0) & 1.95(2.0) & 1.69(4.0) & 1.83(3.0) & 1.97(1.0) & 1.47(5.0)  \\ 
  wal & 2.96(1.0) & 1.69(5.0) & 2.06(3.5) & 2.06(3.5) & 1.49(6.0) & 2.13(2.0)  \\ 
  wa1 & 2.51(4.0) & 2.08(6.0) & 3.38(1.0) & 3.16(2.0) & 2.15(5.0) & 2.55(3.0)  \\ 
  wa2 & 2.35(4.0) & 1.98(6.0) & 3.12(1.0) & 2.96(2.0) & 2.41(3.0) & 2.34(5.0)  \\ 
  win & 3.63(1.0) & 3.29(3.0) & 2.84(6.0) & 3.50(2.0) & 2.90(5.0) & 3.01(4.0)  \\ 
  yea & 2.48(1.5) & 2.09(4.0) & 2.48(1.5) & 2.32(3.0) & 1.90(6.0) & 1.98(5.0)  \\ 
  \hline
  avg & 3.31(2.2) & 2.44(4.59) & 3.18(3.21) & 3.27(2.71) & 2.66(4.47) & 3.16(3.81)  \\ 
 \end{tabular}
 }
 \caption{Augmented AUC scores and ranks using the third hyperparameter selection criterion, using top 1\% of samples.} 
 \label{tab:top1aaucfull} 
\end{table}

==> misc/top5aaucfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 3.52(1.0) & 2.41(5.0) & 3.24(2.0) & 3.18(3.0) & 2.27(6.0) & 2.61(4.0)  \\ 
  blo & 4.15(1.0) & 3.92(2.0) & 3.89(3.0) & 3.81(6.0) & 3.83(5.0) & 3.84(4.0)  \\ 
  brc & 3.38(5.0) & 4.17(1.0) & 3.87(2.0) & 3.78(4.0) & 3.29(6.0) & 3.85(3.0)  \\ 
  brt & 3.45(2.5) & 3.45(2.5) & 3.50(1.0) & 3.28(4.0) & 2.86(6.0) & 2.98(5.0)  \\ 
  car & 1.58(4.0) & 1.40(6.0) & 1.57(5.0) & 1.62(3.0) & 1.90(2.0) & 2.10(1.0)  \\ 
  eco & 3.26(3.0) & 2.20(6.0) & 3.38(1.0) & 3.33(2.0) & 2.49(5.0) & 2.50(4.0)  \\ 
  gla & 2.28(5.0) & 1.84(6.0) & 2.54(4.0) & 2.61(3.0) & 3.01(1.0) & 2.99(2.0)  \\ 
  hab & 3.45(1.0) & 3.14(3.0) & 2.76(5.0) & 3.19(2.0) & 2.79(4.0) & 2.50(6.0)  \\ 
  ion & 3.74(2.0) & 2.90(5.0) & 3.70(3.0) & 3.83(1.0) & 2.72(6.0) & 3.67(4.0)  \\ 
  iri & 3.06(5.0) & 2.29(6.0) & 3.07(4.0) & 3.16(3.0) & 3.55(2.0) & 3.60(1.0)  \\ 
  iso & 2.49(1.0) & 1.42(5.0) & 2.23(3.0) & 2.26(2.0) & 1.39(6.0) & 1.78(4.0)  \\ 
  let & 2.50(1.0) & 1.18(6.0) & 2.36(3.0) & 2.38(2.0) & 1.26(5.0) & 1.91(4.0)  \\ 
  lib & 2.35(1.0) & 1.56(6.0) & 2.16(3.0) & 1.99(4.0) & 1.77(5.0) & 2.19(2.0)  \\ 
  mad & 1.22(4.0) & 1.20(5.0) & 1.17(6.0) & 1.33(2.0) & 1.27(3.0) & 3.21(1.0)  \\ 
  mag & 4.72(1.0) & 3.52(4.0) & 4.11(3.0) & 4.45(2.0) & 2.98(6.0) & 3.28(5.0)  \\ 
  min & 2.33(4.0) & 2.30(5.0) & 2.11(6.0) & 3.62(1.0) & 3.11(3.0) & 3.36(2.0)  \\ 
  mul & 4.66(2.0) & 2.10(6.0) & 4.57(3.0) & 5.22(1.0) & 2.84(5.0) & 4.18(4.0)  \\ 
  mus & 5.91(2.0) & 1.19(6.0) & 5.69(3.0) & 6.00(1.0) & 2.39(5.0) & 4.95(4.0)  \\ 
  pag & 4.55(4.0) & 3.67(5.5) & 5.10(2.0) & 5.28(1.0) & 3.67(5.5) & 4.60(3.0)  \\ 
  par & 2.80(2.0) & 2.14(5.0) & 2.77(3.0) & 2.22(4.0) & 2.06(6.0) & 3.03(1.0)  \\ 
  pen & 6.30(1.0) & 2.98(6.0) & 5.23(3.0) & 5.40(2.0) & 3.41(5.0) & 3.49(4.0)  \\ 
  pim & 2.47(1.0) & 2.38(4.0) & 2.41(2.0) & 2.40(3.0) & 2.07(6.0) & 2.33(5.0)  \\ 
  son & 1.47(4.0) & 1.43(5.0) & 1.37(6.0) & 1.61(3.0) & 3.19(1.0) & 3.14(2.0)  \\ 
  spe & 2.27(2.0) & 1.97(5.5) & 2.47(1.0) & 2.22(3.5) & 1.97(5.5) & 2.22(3.5)  \\ 
  ssa & 4.72(3.0) & 3.91(6.0) & 4.82(2.0) & 4.46(5.0) & 4.61(4.0) & 5.11(1.0)  \\ 
  sse & 4.31(2.0) & 2.94(6.0) & 4.24(3.0) & 3.96(4.0) & 3.75(5.0) & 4.68(1.0)  \\ 
  ssh & 5.77(1.0) & 3.95(5.0) & 4.80(2.0) & 4.50(3.0) & 2.98(6.0) & 4.06(4.0)  \\ 
  sve & 2.51(4.0) & 1.97(6.0) & 2.56(2.0) & 2.71(1.0) & 2.12(5.0) & 2.55(3.0)  \\ 
  syn & 4.72(1.0) & 2.77(6.0) & 3.91(3.0) & 3.86(4.0) & 3.63(5.0) & 4.50(2.0)  \\ 
  ver & 1.82(5.0) & 1.96(2.0) & 1.61(6.0) & 1.91(3.0) & 2.03(1.0) & 1.88(4.0)  \\ 
  wal & 2.96(1.0) & 1.73(5.0) & 2.07(4.0) & 2.10(3.0) & 1.49(6.0) & 2.26(2.0)  \\ 
  wa1 & 2.51(4.0) & 2.12(6.0) & 3.34(1.0) & 3.18(2.0) & 2.37(5.0) & 2.77(3.0)  \\ 
  wa2 & 2.35(5.0) & 2.04(6.0) & 3.09(2.0) & 3.21(1.0) & 2.52(3.5) & 2.52(3.5)  \\ 
  win & 3.68(1.0) & 3.31(5.0) & 2.84(6.0) & 3.50(4.0) & 3.54(3.0) & 3.60(2.0)  \\ 
  yea & 2.48(3.0) & 2.07(6.0) & 2.89(2.0) & 2.99(1.0) & 2.10(5.0) & 2.41(4.0)  \\ 
  \hline
  avg & 3.27(2.56) & 2.44(5.01) & 3.07(3.14) & 3.18(2.67) & 2.41(4.53) & 2.69(3.09)  \\ 
 \end{tabular}
 }
 \caption{Augmented AUC scores and ranks using the third hyperparameter selection criterion, using top 5\% of samples.} 
 \label{tab:top5aaucfull} 
\end{table}

==> misc/trainaaucfull.tex <==
\begin{table} 
 \center 
 \resizebox{\columnwidth}{!}{ 
 \begin{tabular}[h]{c | c c c c c c } 
  dataset & kNN & IForest & AE & VAE & GAN & fmGAN  \\ 
  \hline 
  aba & 3.52(2.0) & 2.41(6.0) & 3.36(4.0) & 3.24(5.0) & 3.40(3.0) & 5.26(1.0)  \\ 
  blo & 4.08(3.5) & 3.92(6.0) & 3.96(5.0) & 4.08(3.5) & 4.32(2.0) & 4.83(1.0)  \\ 
  brc & 3.38(6.0) & 4.30(1.0) & 3.90(3.0) & 3.71(4.0) & 3.63(5.0) & 4.19(2.0)  \\ 
  brt & 3.45(2.5) & 3.45(2.5) & 3.50(1.0) & 3.28(4.0) & 2.86(6.0) & 2.98(5.0)  \\ 
  car & 1.58(5.0) & 1.42(6.0) & 1.67(4.0) & 2.00(3.0) & 2.78(2.0) & 3.08(1.0)  \\ 
  eco & 3.26(4.0) & 2.19(6.0) & 3.32(2.0) & 3.27(3.0) & 2.65(5.0) & 3.61(1.0)  \\ 
  gla & 2.28(5.0) & 1.86(6.0) & 2.54(4.0) & 2.61(3.0) & 3.47(2.0) & 3.58(1.0)  \\ 
  hab & 3.45(2.0) & 3.19(3.0) & 2.76(5.0) & 3.08(4.0) & 2.51(6.0) & 3.96(1.0)  \\ 
  ion & 3.74(3.0) & 2.99(5.5) & 3.70(4.0) & 3.83(2.0) & 2.99(5.5) & 4.00(1.0)  \\ 
  iri & 3.06(5.0) & 2.34(6.0) & 3.12(4.0) & 3.16(3.0) & 3.55(2.0) & 3.60(1.0)  \\ 
  iso & 2.49(1.0) & 1.43(5.0) & 2.08(3.0) & 2.20(2.0) & 1.36(6.0) & 1.89(4.0)  \\ 
  let & 2.50(1.0) & 1.18(6.0) & 2.29(2.0) & 2.24(3.0) & 1.39(5.0) & 1.89(4.0)  \\ 
  lib & 2.35(1.0) & 1.59(6.0) & 2.16(4.0) & 1.99(5.0) & 2.29(2.0) & 2.19(3.0)  \\ 
  mad & 1.22(4.5) & 1.22(4.5) & 1.17(6.0) & 1.33(3.0) & 1.34(2.0) & 2.66(1.0)  \\ 
  mag & 4.72(2.0) & 3.52(6.0) & 4.19(5.0) & 4.44(4.0) & 4.60(3.0) & 6.20(1.0)  \\ 
  min & 2.33(4.0) & 2.30(5.0) & 2.17(6.0) & 3.72(1.0) & 3.21(3.0) & 3.52(2.0)  \\ 
  mul & 4.66(2.0) & 2.16(6.0) & 4.57(3.0) & 5.22(1.0) & 2.67(5.0) & 4.05(4.0)  \\ 
  mus & 5.91(2.0) & 1.22(6.0) & 5.84(3.0) & 6.08(1.0) & 3.01(5.0) & 5.12(4.0)  \\ 
  pag & 4.55(4.0) & 3.67(6.0) & 5.11(3.0) & 5.21(2.0) & 4.32(5.0) & 6.88(1.0)  \\ 
  par & 2.80(2.0) & 2.16(6.0) & 2.77(3.0) & 2.22(5.0) & 2.75(4.0) & 2.95(1.0)  \\ 
  pen & 6.30(1.0) & 2.99(6.0) & 5.31(3.0) & 5.54(2.0) & 4.09(5.0) & 5.10(4.0)  \\ 
  pim & 2.47(4.0) & 2.39(5.0) & 2.48(3.0) & 2.28(6.0) & 3.11(2.0) & 4.26(1.0)  \\ 
  son & 1.47(4.0) & 1.42(5.0) & 1.37(6.0) & 1.61(3.0) & 3.27(1.0) & 2.99(2.0)  \\ 
  spe & 2.27(2.0) & 1.97(6.0) & 2.44(1.0) & 2.21(4.0) & 2.07(5.0) & 2.22(3.0)  \\ 
  ssa & 4.72(3.0) & 3.98(6.0) & 4.79(2.0) & 4.60(4.0) & 4.50(5.0) & 5.22(1.0)  \\ 
  sse & 4.31(2.0) & 2.97(6.0) & 4.11(4.0) & 4.23(3.0) & 3.56(5.0) & 4.94(1.0)  \\ 
  ssh & 6.32(2.0) & 4.03(6.0) & 5.82(4.0) & 5.88(3.0) & 4.58(5.0) & 7.52(1.0)  \\ 
  sve & 2.51(5.0) & 1.96(6.0) & 2.71(3.0) & 2.72(2.0) & 2.56(4.0) & 4.06(1.0)  \\ 
  syn & 4.76(1.0) & 2.83(6.0) & 3.79(4.0) & 3.87(3.0) & 3.70(5.0) & 4.51(2.0)  \\ 
  ver & 1.14(6.0) & 1.96(3.0) & 1.61(5.0) & 1.85(4.0) & 2.64(2.0) & 3.95(1.0)  \\ 
  wal & 2.96(2.0) & 1.73(6.0) & 2.08(5.0) & 2.10(4.0) & 2.12(3.0) & 3.48(1.0)  \\ 
  wa1 & 2.51(5.0) & 2.13(6.0) & 3.35(3.0) & 3.31(4.0) & 4.03(2.0) & 4.97(1.0)  \\ 
  wa2 & 2.35(5.0) & 2.04(6.0) & 3.12(4.0) & 3.25(3.0) & 3.83(2.0) & 5.05(1.0)  \\ 
  win & 3.68(3.0) & 3.29(5.0) & 2.84(6.0) & 3.50(4.0) & 3.74(1.0) & 3.69(2.0)  \\ 
  yea & 2.48(5.0) & 2.09(6.0) & 2.65(3.0) & 2.76(2.0) & 2.64(4.0) & 4.42(1.0)  \\ 
  \hline
  avg & 3.27(3.19) & 2.44(5.39) & 3.07(3.71) & 3.18(3.21) & 2.41(3.7) & 2.69(1.8)  \\ 
 \end{tabular}
 }
 \caption{Augmented AUC scores and ranks using the second hyperparameter selection criterion.} 
 \label{tab:trainaaucfull} 
\end{table}
